SemCity: Semantic Scene Generation with Triplane Diffusion

We present "SemCity," a 3D diffusion model for semantic scene generation in real-world outdoor environments. Most 3D diffusion models focus on generating a single object, synthetic indoor scenes, or synthetic outdoor scenes, while the generation of real-world outdoor scenes is rarely addressed. In this paper, we concentrate on generating a real-outdoor scene through learning a diffusion model on a real-world outdoor dataset. In contrast to synthetic data, real-outdoor datasets often contain more empty spaces due to sensor limitations, causing challenges in learning real-outdoor distributions. To address this issue, we exploit a triplane representation as a proxy form of scene distributions to be learned by our diffusion model. Furthermore, we propose a triplane manipulation that integrates seamlessly with our triplane diffusion model. The manipulation improves our diffusion model's applicability in a variety of downstream tasks related to outdoor scene generation such as scene inpainting, scene outpainting, and semantic scene completion refinements. In experimental results, we demonstrate that our triplane diffusion model shows meaningful generation results compared with existing work in a real-outdoor dataset, SemanticKITTI. We also show our triplane manipulation facilitates seamlessly adding, removing, or modifying objects within a scene. Further, it also enables the expansion of scenes toward a city-level scale. Finally, we evaluate our method on semantic scene completion refinements where our diffusion model enhances predictions of semantic scene completion networks by learning scene distribution. Our code is available at https://github.com/zoomin-lee/SemCity.

==> content/figure_tex/figure1.tex <==
\begin{figure*}[t]
\begin{center}
\centerline{\includegraphics[trim={0cm 9.98cm 0.55cm 0cm},clip,width=1.0\linewidth]{figure/intro.pdf}}
   \captionof{figure}{
   We introduce a diffusion framework, \textit{SemCity}, designed for generating semantic scenes in real-world outdoor environments as shown in  $\text{(a)}$.
   We extend our diffusion model to various practical tasks: semantic scene completion refinement, scene outpainting, and scene inpainting.
   For instance, the comprehensive scenario is displayed in $\text{(b)} \! \rightarrow \! \text{(c)} \! \rightarrow \! \text{(d)}$:
   % (c) our diffusion model refines the prediction semantic scene completion result (SSC).
   % (3)
   The refined scene (SSC refinement) $\text{(b)}$ is outpainted to a broader scene $\text{(c)}$; then, an object (in this case, a car) is seamlessly integrated into the scene via our inpainting process $\text{(d)}$.
   }
    \label{fig:intro}
\end{center}
\end{figure*}

==> content/table_tex/carlasc.tex <==
\definecolor{building}{RGB}{255, 200, 0}
\definecolor{barrier}{RGB}{255, 120, 50}
\definecolor{other}{RGB}{55, 90, 80}
\definecolor{pedestrian}{RGB}{255, 30, 30}
\definecolor{pole}{RGB}{255, 240, 150}
\definecolor{road}{RGB}{255, 0, 255}
\definecolor{ground}{RGB}{175, 0, 75}
\definecolor{sidewalk}{RGB}{75, 0, 75}
\definecolor{vegetation}{RGB}{0, 175, 0}
\definecolor{vehicles}{RGB}{100, 150, 245}


\begin{table*}[p]{
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}
{\normalsize
\begin{tabular}{c|cccccccccccc|c}
\hline
 & \multicolumn{12}{c|}{Class IoU} &  \\ \cline{2-13}
\multirow{-2}{*}{} & \multicolumn{1}{c|}{mIoU} & Free & \cellcolor[HTML]{FFC800}Building & \cellcolor[HTML]{FF7832}Barrier & \cellcolor[HTML]{375A50}{\color[HTML]{FFFFFF} Other} & \cellcolor[HTML]{FF1E1E}{\color[HTML]{FFFFFF}Pedestrian} & \cellcolor[HTML]{FFF096}Pole & \cellcolor[HTML]{FF00FF}Road & \cellcolor[HTML]{AF004B}{\color[HTML]{FFFFFF} Ground} & \cellcolor[HTML]{4B004B}{\color[HTML]{FFFFFF} Sidewalk} & \cellcolor[HTML]{00AF00}Vegetation & \cellcolor[HTML]{6496F5}Vehicles & \multirow{-2}{*}{IoU} \\ \hline
w/o Diffusion & \multicolumn{1}{c|}{39.94} & 96.40 & 27.72 & 3.15 & 8.77 & 22.15 & 37.14 & \textbf{89.02} & \textbf{18.22} & 59.25 & 29.74 & 47.72 & 80.70 \\
Discrete Diffusion (Ours) & \multicolumn{1}{c|}{\textbf{45.83}} & 96.00 & \textbf{31.75} & 3.42 & \textbf{25.43} & \textbf{46.22} & \textbf{43.32} & 84.57 & 13.01 & \textbf{67.50} & \textbf{37.45} & \textbf{55.46} & 80.61 \\ \hline
\end{tabular}
}
}
\caption{\textbf{Semantic scene completion results} on test set of CarlaSC. The discriminative learning result with the diffusion model architecture is denoted as `w/o Diffusion'. %To compare meaningful results, 
Values with a difference equal to or greater than 0.5\%p are bold.}
\label{tab:ours}
\end{table*}

==> content/table_tex/kitti.tex <==
\definecolor{car}{RGB}{100, 120, 245}
\definecolor{bicycle}{RGB}{50, 230, 255}
\definecolor{motorcycle}{RGB}{30, 60, 150}
\definecolor{truck}{RGB}{80, 30, 180}
\definecolor{other-vehicle}{RGB}{0, 0, 255}
\definecolor{person}{RGB}{255, 30, 30}
\definecolor{bicyclist}{RGB}{255, 40, 200}
\definecolor{motorcyclist}{RGB}{150, 30, 90}
\definecolor{road}{RGB}{255, 0, 255}
\definecolor{parking}{RGB}{255, 150, 255}
\definecolor{sidewalk}{RGB}{75, 0, 75}
\definecolor{other-ground}{RGB}{175, 0, 75}
\definecolor{building}{RGB}{255, 200, 0}
\definecolor{fence}{RGB}{255, 120, 50}
\definecolor{vegetation}{RGB}{0, 175, 0}
\definecolor{trunk}{RGB}{135, 60, 0}
\definecolor{terrain}{RGB}{150, 240, 80}
\definecolor{pole}{RGB}{255, 240, 150}
\definecolor{traffic-sign}{RGB}{255, 0, 0}
\begin{table*}[]
\centering\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{c|c|ccccccccccccccccccc|c}

\hline
               & SC  & \multicolumn{19}{c|}{SSC}                                                                                                                                                                             &      \\
Method         & IoU & \rotatebox{90}{{\textcolor{road}{$\blacksquare$}}~road} & \rotatebox{90}{{\textcolor{sidewalk}{$\blacksquare$}}~sidewalk} & \rotatebox{90}{{\textcolor{parking}{$\blacksquare$}}~parking} & \rotatebox{90}{{\textcolor{other-ground}{$\blacksquare$}}~other-ground} & \rotatebox{90}{{\textcolor{building}{$\blacksquare$}}~building} & \rotatebox{90}{{\textcolor{car}{$\blacksquare$}}~car} & \rotatebox{90}{{\textcolor{truck}{$\blacksquare$}}~truck} & \rotatebox{90}{{\textcolor{bicycle}{$\blacksquare$}}~bicycle} & \rotatebox{90}{{\textcolor{motorcycle}{$\blacksquare$}}~motorcycle} & \rotatebox{90}{{\textcolor{other-vehicle}{$\blacksquare$}}~other-vehicle} & \rotatebox{90}{{\textcolor{vegetation}{$\blacksquare$}}~vegetation} & \rotatebox{90}{{\textcolor{trunk}{$\blacksquare$}}~trunk} & \rotatebox{90}{{\textcolor{terrain}{$\blacksquare$}}~terrain} & \rotatebox{90}{{\textcolor{person}{$\blacksquare$}}~person} & \rotatebox{90}{{\textcolor{bicyclist}{$\blacksquare$}}~bicyclist} & \rotatebox{90}{{\textcolor{motorcyclist}{$\blacksquare$}}~motorcyclist} & \rotatebox{90}{{\textcolor{fence}{$\blacksquare$}}~fence} & \rotatebox{90}{{\textcolor{pole}{$\blacksquare$}}~pole} & \rotatebox{90}{{\textcolor{traffic-sign}{$\blacksquare$}}~traffic-sign} & mIoU \\ \hline
MonoScene~\cite{cao2022monoscene}      & 37.12 & 57.47 & 27.05    & 15.72   & 0.87         & 14.24    & 23.55 & 7.83  & 0.20    & 0.77       & 3.59          & 18.12      & 2.57  & 30.76   & 1.79   & 1.03      & 0.00         & 6.39  & 4.11 & 2.48         & 11.50  \\
MonoScene+Ours &     &      &          &         &              &          &     &       &         &            &           &            &       &         &        &           &              &       &      &              &      \\ \hline
OccDepth~\cite{miao2023occdepth}       &   41.60 &  56.50          & 25.68          & 12.37          & \textbf{0.74} & 19.21          & 27.49          & \textbf{6.08} & \textbf{0.44} & \textbf{1.33} & \textbf{4.56} & 23.59          & \textbf{7.68} & 32.14          & \textbf{1.83} & \textbf{0.88} & 0.00         & 6.97          & \textbf{10.56} & \textbf{5.85}  &  12.84 \\
OccDepth+Ours &     &      &          &         &              &          &     &       &         &            &           &            &       &         &        &           &              &       &      &              &      \\ \hline
SCPNet & 50.24 & 70.75 & 53.04    & 61.54   & 15.13        & 33.56    & 51.15 & 57.58 & 25.82   & 37.68      & 43.83         & 38.85      & 33.86 & 52.88   & 22.91  & 18.77     & 4.18         & 32.21 & 39.80 & 19.79 & 37.55 \\ 
SCPNet+Ours &     &      &          &         &              &          &     &       &         &            &           &            &       &         &        &           &              &       &      &              &      \\ \hline
\end{tabular}}
\caption{Semantic scene completion refinement quantitative results on SemanticKITTI~\cite{semantickitti}}

\end{table*}



==> content/table_tex/table0.tex <==
\definecolor{car}{RGB}{100, 120, 245}
\definecolor{bicycle}{RGB}{50, 230, 255}
\definecolor{motorcycle}{RGB}{30, 60, 150}
\definecolor{truck}{RGB}{80, 30, 180}
\definecolor{other-vehicle}{RGB}{0, 0, 255}
\definecolor{person}{RGB}{255, 30, 30}
\definecolor{bicyclist}{RGB}{255, 40, 200}
\definecolor{motorcyclist}{RGB}{150, 30, 90}
\definecolor{road}{RGB}{255, 0, 255}
\definecolor{parking}{RGB}{255, 150, 255}
\definecolor{sidewalk}{RGB}{75, 0, 75}
\definecolor{other-ground}{RGB}{175, 0, 75}
\definecolor{building}{RGB}{255, 200, 0}
\definecolor{fence}{RGB}{255, 120, 50}
\definecolor{vegetation}{RGB}{0, 175, 0}
\definecolor{trunk}{RGB}{135, 60, 0}
\definecolor{terrain}{RGB}{150, 240, 80}
\definecolor{pole}{RGB}{255, 240, 150}
\definecolor{traffic-sign}{RGB}{255, 0, 0}

\begin{table*}[]
\small
\begin{tabular}{cccccccccc}
{{\textcolor{road}{$\blacksquare$}}~road} & {{\textcolor{sidewalk}{$\blacksquare$}}~sidewalk} & {{\textcolor{parking}{$\blacksquare$}}~parking} & {{\textcolor{other-ground}{$\blacksquare$}}~ground} & {{\textcolor{building}{$\blacksquare$}}~building} & {{\textcolor{traffic-sign}{$\blacksquare$}}~traffic-sign}  & {{\textcolor{truck}{$\blacksquare$}}~truck} &{{\textcolor{bicycle}{$\blacksquare$}}~bicycle} & \multicolumn{2}{l}{{\textcolor{motorcycle}{$\blacksquare$}}~motorcycle} 
{{\textcolor{other-vehicle}{$\blacksquare$}}~vehicle}&{{\textcolor{vegetation}{$\blacksquare$}}~vegetation} & {{\textcolor{trunk}{$\blacksquare$}}~trunk} & {{\textcolor{terrain}{$\blacksquare$}}~terrain} &{{\textcolor{person}{$\blacksquare$}}~person} & {{\textcolor{bicyclist}{$\blacksquare$}}~bicyclist} & {{\textcolor{motorcyclist}{$\blacksquare$}}~motorcyclist} & {{\textcolor{fence}{$\blacksquare$}}~fence} & {{\textcolor{pole}{$\blacksquare$}}~pole} & 
{{\textcolor{car}{$\blacksquare$}}~car}
\end{tabular}
\end{table*}

==> content/table_tex/table_carla_ssc_results.tex <==
\begin{table}[]
\begin{center}
\small{
\begin{tabular}{lcc}
\hline
Method         & IoU $\uparrow$ & mIoU $\uparrow$ \\ \hline
SSCNet~\cite{song2017semantic} & 80.69  & 41.91   \\
SSCNet + Ours & 84.37 & 43.56 \\ \hline
LMSCNet~\cite{roldao2020lmscnet} & 85.98 &  42.53  \\
LMSCNet + Ours & & \\ \hline
MotionSC\cite{carlasc} &  86.46 & 46.31   \\
MotionSC + Ours & 87.10 &  46.80 \\ \hline
\end{tabular}
\caption{
    \textbf{Quantitative results of refining SSC predictions on CarlaSC test set~\cite{carlasc}.}
}\label{tab:carla_refine}
}
\end{center}
\end{table}

==> preamble.tex <==
%
% --- inline annotations
\usepackage{siunitx}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{kotex}
\usepackage{verbatim}
\usepackage{amssymb}
\usepackage[table,xcdraw]{xcolor}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}


